Measuring Orthogonality in Representations of Generative Models

In unsupervised representation learning, models aim to distill essential features from high-dimensional data into lower-dimensional learned representations, guided by inductive biases. Understanding the characteristics that make a good representation remains a topic of ongoing research. Disentanglement of independent generative processes has long been credited with producing high-quality representations. However, focusing solely on representations that adhere to the stringent requirements of most disentanglement metrics, may result in overlooking many high-quality representations, well suited for various downstream tasks. These metrics often demand that generative factors be encoded in distinct, single dimensions aligned with the canonical basis of the representation space. Motivated by these observations, we propose two novel metrics: Importance-Weighted Orthogonality (IWO) and Importance-Weighted Rank (IWR). These metrics evaluate the mutual orthogonality and rank of generative factor subspaces. Throughout extensive experiments on common downstream tasks, over several benchmark datasets and models, IWO and IWR consistently show stronger correlations with downstream task performance than traditional disentanglement metrics. Our findings suggest that representation quality is closer related to the orthogonality of independent generative processes rather than their disentanglement, offering a new direction for evaluating and improving unsupervised learning models.

==> gradient.tex <==
% Siavoosh Payandeh Azad Jan. 2019
\ProvidesPackage{highlight}[Cell background highlighting based on user data]
\RequirePackage{etoolbox}
\RequirePackage{pgf} % for calculating the values for gradient
\RequirePackage{xcolor} % enables the use of cellcolor make sure you have [table] option in the document class 
% Color set related!
% Color set related!
\definecolor{high}{HTML}{77DD77}  % the color for the highest number in your data set
\definecolor{low}{HTML}{fff7bc}  % the color for the lowest number in your data set
\newcommand*{\opacity}{90}% here you can change the opacity of the background color!
%======================================
% Data set related!
\newcommand*{\minval}{0.0}% define the minimum value on your data set
\newcommand*{\maxval}{1.0}% define the maximum value in your data set!
\newcommand*{\minvalz}{0.5}% define the minimum value on your data set
\newcommand*{\maxvalz}{1.0}% define the maximum value in your data set!
%======================================
% gradient function!
\newcommand{\gradient}[1]{
    % The values are calculated linearly between \minval and \maxval
    \ifdimcomp{#1pt}{>}{\maxval pt}{#1}{
    \ifdimcomp{#1pt}{<}{\minval pt}{#1}{
         \pgfmathparse{int(round(100*(#1/(\maxval-\minval))-(\minval*(100/(\maxval-\minval)))))}
        \xdef\tempa{\pgfmathresult}
        \cellcolor{high!\tempa!low!\opacity} #1
    }}
 }
 \newcommand{\gradientb}[1]{
    % The values are calculated linearly between \minval and \maxval
    \ifdimcomp{#1pt}{>}{\maxval pt}{#1}{
    \ifdimcomp{#1pt}{<}{\minval pt}{#1}{
         \pgfmathparse{int(round(100*(#1/(\maxval-\minval))-(\minval*(100/(\maxval-\minval)))))}
        \xdef\tempa{\pgfmathresult}
        \cellcolor{high!\tempa!low!\opacity} \textbf{#1}
    }}
 }
\newcommand{\gradientz}[1]{
    % The values are calculated linearly between \minval and \maxval
    \ifdimcomp{#1pt}{>}{\maxvalz pt}{#1}{
    \ifdimcomp{#1pt}{<}{\minvalz pt}{#1}{
         \pgfmathparse{int(round(100*(#1/(\maxvalz-\minvalz))-(\minvalz*(100/(\maxvalz-\minvalz)))))}
        \xdef\tempa{\pgfmathresult}
        \cellcolor{high!\tempa!low!\opacity} #1
    }}
 }

 % Color set related!
\definecolor{highn}{HTML}{fff7bc}  % the color for the highest number in your data set
\definecolor{lown}{HTML}{ef3b2c}  % the color for the lowest number in your data set
%======================================
% Data set related!
\newcommand*{\minvaln}{-1.0}% define the minimum value on your data set
\newcommand*{\maxvaln}{0.0}% define the maximum value in your data set!
%======================================
% gradient function!
\newcommand{\gradientn}[1]{
    % The values are calculated linearly between \minval and \maxval
    \ifdimcomp{#1pt}{>}{\maxvaln pt}{#1}{
    \ifdimcomp{#1pt}{<}{\minvaln pt}{#1}{
         \pgfmathparse{int(round(100*(#1/(\maxvaln-\minvaln))-(\minvaln*(100/(\maxvaln-\minvaln)))))}
        \xdef\tempa{\pgfmathresult}
        \cellcolor{highn!\tempa!lown!\opacity} #1
    }}
 }

% Data set related!
%======================================
% Data set related!
\newcommand*{\minvalnz}{0.0}% define the minimum value on your data set
\newcommand*{\maxvalnz}{0.5}% define the maximum value in your data set!
%======================================
% gradient function!
\newcommand{\gradientnz}[1]{
    % The values are calculated linearly between \minval and \maxval
    \ifdimcomp{#1pt}{>}{\maxvalnz pt}{#1}{
    \ifdimcomp{#1pt}{<}{\minvalnz pt}{#1}{
         \pgfmathparse{int(round(100*(#1/(\maxvalnz-\minvalnz))-(\minvalnz*(100/(\maxvalnz-\minvalnz)))))}
        \xdef\tempa{\pgfmathresult}
        \cellcolor{highn!\tempa!lown!\opacity} #1
    }}
 }

==> tables/all_exps.tex <==
\begin{table}[h!]
\caption{Individual correlations between metrics and downstream task (DST) performance. Each model is trained on six different datasets. For each dataset, six different hyperparameters on 10 random seeds are trained for a total of 2160 learned representations. Correlations between downstream task performance and the three commonly used metrics DCI-D, DCI-C and MIG together with IWO and IWR are calculated. Correlations are calculated between averaged task performance and averaged metrics, where the average is taken over the seeds and grouped by hyperparameter. As such, we assess the capability of the metrics to point us to good models and hyperparameters. }
\label{tab:all_exps}
\centering
\scriptsize
\setlength{\tabcolsep}{0.3pt} 
\renewcommand{\arraystretch}{1}
\begin{tabular}{ll|ccccc|ccccc|ccccc}
\toprule
& & \multicolumn{5}{c}{Random Forest} & \multicolumn{5}{c}{Logistic Regression} & \multicolumn{5}{c}{Neural Network} \\
\midrule
 & & D & C & MIG & IWO & IWR  & D & C & MIG & IWO & IWR  & D & C & MIG & IWO & IWR \\
 \midrule
\multirow{6}{*}{\begin{turn}{90}Cars3D\end{turn}} & AnnealedVAE & \gradient{0.72} & \gradientn{-0.18} & \gradientn{-0.19} & \gradient{0.74} & \gradient{0.69} & \gradientn{-0.40} & \gradientn{-0.85} & \gradientn{-0.82} & \gradient{0.84} & \gradient{0.89} & \gradient{0.25} & \gradientn{-0.36} & \gradientn{-0.33} & \gradient{0.98} & \gradient{0.97} \\
 & $\beta$-TCVAE & \gradientn{-0.92} & \gradientn{-0.91} & \gradientn{-0.91} & \gradient{0.80} & \gradient{0.11} & \gradientn{-0.94} & \gradientn{-0.97} & \gradientn{-0.90} & \gradient{0.75} & \gradientn{-0.15} & \gradient{0.06} & \gradientn{-0.04} & \gradient{0.16} & \gradientn{-0.48} & \gradientn{-0.90} \\
 & $\beta$-VAE & \gradientn{-0.92} & \gradientn{-0.94} & \gradientn{-0.93} & \gradient{0.67} & \gradient{0.80} & \gradientn{-0.93} & \gradientn{-0.95} & \gradientn{-0.92} & \gradient{0.60} & \gradient{0.91} & \gradientn{-0.66} & \gradientn{-0.67} & \gradientn{-0.67} & \gradient{0.22} & \gradient{0.82} \\
 & DIP-VAE-I & \gradientn{-0.84} & \gradientn{-0.77} & \gradientn{-0.61} & \gradientn{-0.09} & \gradientn{-0.18} & \gradient{0.61} & \gradient{0.39} & \gradientn{-0.10} & \gradient{0.68} & \gradient{0.73} & \gradientn{-0.07} & \gradientn{-0.32} & \gradientn{-0.50} & \gradient{0.98} & \gradient{0.99} \\
 & DIP-VAE-II & \gradientn{-0.89} & \gradientn{-0.96} & \gradientn{-0.76} & \gradient{0.90} & \gradient{0.59} & \gradientn{-0.49} & \gradientn{-0.72} & \gradientn{-0.74} & \gradient{0.74} & \gradient{0.83} & \gradientn{-0.49} & \gradientn{-0.70} & \gradientn{-0.49} & \gradient{0.67} & \gradient{0.94} \\
 & FactorVAE & \gradientn{-0.26} & \gradientn{-0.17} & \gradientn{-0.81} & \gradient{0.78} & \gradient{0.74} & \gradientn{-0.17} & \gradientn{-0.31} & \gradientn{-0.71} & \gradient{0.91} & \gradient{0.91} & \gradient{0.22} & \gradientn{-0.08} & \gradientn{-0.49} & \gradient{0.97} & \gradient{0.98} \\
\cline{1-17}
\multirow{6}{*}{\begin{turn}{90}Color DSprites\end{turn}} & AnnealedVAE & \gradient{1.00} & \gradient{1.00} & \gradient{0.98} & \gradient{0.97} & \gradient{0.97} & \gradient{0.86} & \gradient{0.85} & \gradient{0.90} & \gradient{0.91} & \gradient{0.94} & \gradientn{-0.80} & \gradientn{-0.80} & \gradientn{-0.82} & \gradientn{-0.86} & \gradientn{-0.85} \\
 & $\beta$-TCVAE & \gradient{0.99} & \gradient{0.99} & \gradient{1.00} & \gradient{0.78} & \gradient{0.97} & \gradient{0.44} & \gradient{0.54} & \gradient{0.45} & \gradient{0.70} & \gradient{0.55} & \gradientn{-0.81} & \gradientn{-0.89} & \gradientn{-0.85} & \gradientn{-0.68} & \gradientn{-0.86} \\
 & $\beta$-VAE & \gradient{0.98} & \gradient{0.99} & \gradient{1.00} & \gradientn{-0.80} & \gradient{0.76} & \gradient{0.69} & \gradient{0.85} & \gradient{0.80} & \gradientn{-0.45} & \gradient{0.93} & \gradientn{-0.67} & \gradientn{-0.85} & \gradientn{-0.78} & \gradient{0.32} & \gradientn{-0.95} \\
 & DIP-VAE-I & \gradient{0.46} & \gradient{0.39} & \gradient{0.61} & \gradient{0.96} & \gradient{0.94} & \gradient{0.73} & \gradient{0.68} & \gradient{0.70} & \gradient{0.78} & \gradient{0.63} & \gradient{0.89} & \gradient{0.91} & \gradient{0.75} & \gradient{0.04} & \gradientn{-0.18} \\
 & DIP-VAE-II & \gradient{0.07} & \gradient{0.50} & \gradientn{-0.07} & \gradientn{-0.73} & \gradient{0.26} & \gradient{0.37} & \gradientn{-0.78} & \gradient{0.39} & \gradient{0.90} & \gradientn{-0.81} & \gradient{0.71} & \gradientn{-0.45} & \gradient{0.73} & \gradient{0.50} & \gradientn{-0.92} \\
 & FactorVAE & \gradient{0.91} & \gradient{0.85} & \gradient{0.63} & \gradient{0.81} & \gradient{0.75} & \gradient{0.86} & \gradient{0.86} & \gradient{0.62} & \gradient{0.82} & \gradient{0.72} & \gradientn{-0.79} & \gradientn{-0.80} & \gradientn{-0.60} & \gradientn{-0.80} & \gradientn{-0.87} \\
\cline{1-17}
\multirow{6}{*}{\begin{turn}{90}DSprites\end{turn}} & AnnealedVAE & \gradient{0.99} & \gradient{0.99} & \gradient{0.97} & \gradient{0.89} & \gradient{0.89} & \gradient{0.84} & \gradient{0.82} & \gradient{0.85} & \gradient{0.87} & \gradient{0.87} & \gradient{0.47} & \gradient{0.45} & \gradient{0.54} & \gradient{0.73} & \gradient{0.72} \\
 & $\beta$-TCVAE & \gradient{1.00} & \gradient{0.99} & \gradient{0.99} & \gradient{0.92} & \gradient{0.97} & \gradient{0.37} & \gradient{0.38} & \gradient{0.25} & \gradient{0.66} & \gradient{0.54} & \gradientn{-0.14} & \gradientn{-0.18} & \gradientn{-0.25} & \gradient{0.07} & \gradient{0.03} \\
 & $\beta$-VAE & \gradient{0.98} & \gradient{0.99} & \gradient{0.97} & \gradient{0.75} & \gradient{0.96} & \gradient{0.03} & \gradient{0.07} & \gradient{0.01} & \gradientn{-0.18} & \gradient{0.02} & \gradientn{-0.04} & \gradientn{-0.06} & \gradient{0.02} & \gradient{0.40} & \gradient{0.08} \\
 & DIP-VAE-I & \gradient{0.96} & \gradient{0.96} & \gradient{0.94} & \gradient{0.28} & \gradient{0.11} & \gradient{0.80} & \gradient{0.79} & \gradient{0.77} & \gradient{0.44} & \gradient{0.35} & \gradient{0.91} & \gradient{0.91} & \gradient{0.90} & \gradientn{-0.10} & \gradientn{-0.22} \\
 & DIP-VAE-II & \gradient{0.77} & \gradient{0.88} & \gradient{0.80} & \gradientn{-0.33} & \gradient{0.93} & \gradientn{-0.20} & \gradientn{-0.46} & \gradientn{-0.43} & \gradient{0.69} & \gradientn{-0.59} & \gradientn{-0.92} & \gradientn{-1.00} & \gradientn{-0.92} & \gradient{0.14} & \gradientn{-0.98} \\
 & FactorVAE & \gradient{0.96} & \gradient{0.94} & \gradient{0.96} & \gradient{0.81} & \gradient{0.86} & \gradient{0.43} & \gradient{0.48} & \gradient{0.35} & \gradient{0.99} & \gradient{0.98} & \gradient{0.79} & \gradient{0.93} & \gradient{0.49} & \gradient{0.86} & \gradient{0.84} \\
\cline{1-17}
\multirow{6}{*}{\begin{turn}{90}Scream DSprites\end{turn}} & AnnealedVAE & \gradient{0.84} & \gradient{0.79} & \gradient{0.85} & \gradient{0.86} & \gradient{0.87} & \gradient{0.92} & \gradient{0.85} & \gradient{0.95} & \gradient{0.92} & \gradient{0.91} & \gradient{0.81} & \gradient{0.86} & \gradient{0.71} & \gradient{0.84} & \gradient{0.84} \\
 & $\beta$-TCVAE & \gradient{0.91} & \gradient{0.98} & \gradient{0.90} & \gradient{0.32} & \gradientn{-0.12} & \gradient{0.93} & \gradient{0.83} & \gradient{0.94} & \gradient{0.65} & \gradientn{-0.46} & \gradientn{-0.88} & \gradientn{-0.75} & \gradientn{-0.89} & \gradientn{-0.78} & \gradient{0.37} \\
 & $\beta$-VAE & \gradient{0.94} & \gradient{0.97} & \gradient{0.96} & \gradient{0.53} & \gradient{0.54} & \gradient{0.86} & \gradient{0.83} & \gradient{0.89} & \gradient{0.78} & \gradient{0.79} & \gradient{0.17} & \gradient{0.13} & \gradient{0.23} & \gradient{0.87} & \gradient{0.90} \\
 & DIP-VAE-I & \gradient{0.79} & \gradient{1.00} & \gradient{0.28} & \gradient{0.68} & \gradient{0.78} & \gradient{0.83} & \gradient{0.50} & \gradient{0.94} & \gradient{0.95} & \gradient{0.89} & \gradient{0.86} & \gradient{0.61} & \gradient{0.89} & \gradient{0.98} & \gradient{0.94} \\
 & DIP-VAE-II & \gradient{0.93} & \gradient{0.92} & \gradient{0.81} & \gradient{0.42} & \gradient{0.46} & \gradient{0.53} & \gradient{0.13} & \gradient{0.76} & \gradient{0.99} & \gradient{1.00} & \gradient{0.49} & \gradient{0.03} & \gradient{0.72} & \gradient{0.99} & \gradient{0.99} \\
 & FactorVAE & \gradient{0.87} & \gradient{0.92} & \gradient{0.80} & \gradient{0.23} & \gradient{0.11} & \gradient{0.65} & \gradient{0.14} & \gradient{0.68} & \gradient{0.79} & \gradient{0.89} & \gradientn{-0.38} & \gradientn{-0.79} & \gradientn{-0.30} & \gradient{0.66} & \gradient{0.64} \\
\cline{1-17}
\multirow{6}{*}{\begin{turn}{90}Shapes3D\end{turn}}& AnnealedVAE & \gradient{0.95} & \gradient{0.62} & \gradient{0.21} & \gradient{0.91} & \gradient{0.96} & \gradient{0.60} & \gradientn{-0.13} & \gradientn{-0.51} & \gradient{0.91} & \gradient{0.83} & \gradient{0.87} & \gradient{0.45} & \gradientn{-0.01} & \gradient{0.97} & \gradient{1.00} \\
 & $\beta$-TCVAE & \gradient{1.00} & \gradient{0.99} & \gradient{0.93} & \gradient{0.90} & \gradient{0.96} & \gradientn{-0.91} & \gradientn{-0.93} & \gradientn{-0.96} & \gradientn{-0.87} & \gradientn{-0.87} & \gradientn{-0.64} & \gradientn{-0.68} & \gradientn{-0.83} & \gradientn{-0.69} & \gradientn{-0.60} \\
 & $\beta$-VAE & \gradient{0.99} & \gradient{0.97} & \gradient{0.86} & \gradientn{-0.57} & \gradient{0.92} & \gradientn{-0.53} & \gradientn{-0.62} & \gradientn{-0.80} & \gradient{0.94} & \gradientn{-0.55} & \gradientn{-0.57} & \gradientn{-0.66} & \gradientn{-0.84} & \gradient{0.92} & \gradientn{-0.63} \\
 & DIP-VAE-I & \gradient{1.00} & \gradient{1.00} & \gradient{0.95} & \gradientn{-0.24} & \gradientn{-0.24} & \gradient{0.46} & \gradient{0.45} & \gradient{0.32} & \gradient{0.57} & \gradient{0.25} & \gradientn{-0.33} & \gradientn{-0.34} & \gradientn{-0.41} & \gradient{0.96} & \gradient{0.82} \\
 & DIP-VAE-II & \gradient{0.99} & \gradient{0.99} & \gradient{0.97} & \gradientn{-0.74} & \gradient{0.74} & \gradientn{-0.63} & \gradientn{-0.78} & \gradientn{-0.83} & \gradient{0.98} & \gradientn{-0.44} & \gradientn{-0.73} & \gradientn{-0.86} & \gradientn{-0.90} & \gradient{0.97} & \gradientn{-0.56} \\
 & FactorVAE & \gradient{0.35} & \gradientn{-0.02} & \gradient{0.03} & \gradient{0.49} & \gradient{0.44} & \gradientn{-0.80} & \gradientn{-0.96} & \gradientn{-0.90} & \gradient{0.59} & \gradient{0.43} & \gradientn{-0.85} & \gradientn{-0.98} & \gradientn{-0.96} & \gradient{0.45} & \gradient{0.27} \\
\cline{1-17}
\multirow{6}{*}{\begin{turn}{90}SmallNorb\end{turn}} & AnnealedVAE & \gradientn{-0.04} & \gradient{0.28} & \gradient{0.77} & \gradient{0.09} & \gradient{0.56} & \gradientn{-0.26} & \gradientn{-0.37} & \gradient{0.21} & \gradient{0.14} & \gradient{0.68} & \gradient{0.50} & \gradient{0.42} & \gradient{0.38} & \gradientn{-0.17} & \gradient{0.80} \\
 & $\beta$-TCVAE & \gradient{0.97} & \gradient{0.76} & \gradient{0.98} & \gradient{0.94} & \gradient{0.99} & \gradient{0.86} & \gradient{0.53} & \gradient{0.97} & \gradient{0.78} & \gradient{0.92} & \gradient{0.93} & \gradient{0.64} & \gradient{1.00} & \gradient{0.89} & \gradient{0.99} \\
 & $\beta$-VAE & \gradient{0.92} & \gradient{0.93} & \gradient{0.97} & \gradient{0.97} & \gradient{1.00} & \gradient{0.97} & \gradient{0.96} & \gradient{0.96} & \gradient{0.93} & \gradient{0.97} & \gradient{0.93} & \gradient{0.94} & \gradient{0.97} & \gradient{0.97} & \gradient{0.99} \\
 & DIP-VAE-I & \gradient{1.00} & \gradient{0.98} & \gradient{0.95} & \gradient{0.97} & \gradient{0.98} & \gradient{0.97} & \gradient{0.94} & \gradient{0.91} & \gradient{0.93} & \gradient{0.94} & \gradient{0.99} & \gradient{0.98} & \gradient{0.96} & \gradient{0.97} & \gradient{0.98} \\
 & DIP-VAE-II & \gradient{0.91} & \gradientn{-0.44} & \gradient{0.88} & \gradient{1.00} & \gradient{0.99} & \gradient{0.85} & \gradientn{-0.56} & \gradient{0.90} & \gradient{0.99} & \gradient{0.98} & \gradient{0.93} & \gradientn{-0.45} & \gradient{0.86} & \gradient{1.00} & \gradient{1.00} \\
 & FactorVAE & \gradient{0.89} & \gradient{0.73} & \gradientn{-0.55} & \gradient{0.95} & \gradient{0.79} & \gradientn{-0.14} & \gradientn{-0.51} & \gradient{0.40} & \gradient{0.13} & \gradient{0.18} & \gradient{0.77} & \gradient{0.59} & \gradientn{-0.47} & \gradient{0.94} & \gradient{0.77} \\
\cline{1-17}
\bottomrule
\end{tabular}
\end{table}
